Buffer is All You Need: Defending Federated Learning against Backdoor Attacks under Non-iids via Buffering

Federated Learning (FL) is a popular paradigm enabling clients to jointly train a global model without sharing raw data. However, FL is known to be vulnerable towards backdoor attacks due to its distributed nature. As participants, attackers can upload model updates that effectively compromise FL. What's worse, existing defenses are mostly designed under independent-and-identically-distributed (iid) settings, hence neglecting the fundamental non-iid characteristic of FL. Here we propose FLBuff for tackling backdoor attacks even under non-iids. The main challenge for such defenses is that non-iids bring benign and malicious updates closer, hence harder to separate. FLBuff is inspired by our insight that non-iids can be modeled as omni-directional expansion in representation space while backdoor attacks as uni-directional. This leads to the key design of FLBuff, i.e., a supervised-contrastive-learning model extracting penultimate-layer representations to create a large in-between buffer layer. Comprehensive evaluations demonstrate that FLBuff consistently outperforms state-of-the-art defenses.

==> 5-discussion.tex <==
\section{Discussions}
\label{sec:discussion}
% Asides from that there are less popular \NIID types \FB has not been applied to, we further discuss two directions for improving \FB.%\xlnote{Could be moved to the appendix.}
% \subsection{Unsupervised and/or Semi-supervised Models}
% Given that currently \FB requires a labelled set for training, therefore it is of practical use to look into converting \FB into an unsupervised or semi-supervised method. One potential approach is to employ unsupervised contrastive learning~\cite{chen2020simple,radford2021learning} to train a self-supervised model that identifies malicious model updates through anomaly detection. While some research has explored this direction~\cite{yang2021cade,fergusonefficient,bansal2023cleanclip}, their applicability on \NIIDs in FL remains unknown and difficult to predict as well. On the contrary, we consider model distillation~\cite{gou2021knowledge} may be a promising technique for this purpose. Recent studies~\cite{zhu2023adfl,zhang2024badcleaner} have used model distillation to create robust student models that inherit the defense capabilities of the corresponding teacher model against backdoor attacks. We plan to look into this direction.


% \subsection{Buffer Layer}
% % We expect that better representation learning is beneficial for obtaining a more viable buffer layer for \FB. A potential direction is considering multiple layers of the model not only the PLRs.
% We view the design of buffer layer as another key direction for improving \FB. One possibility is to use enhanced representation learning to improve the effectiveness of the buffer layer in \FB. For instance, existing work~\cite{CrowdGuard,MESAS,wang2019neural,wang2019neural} found that representation learning from multiple layers rather than PLRs only can strengthen defenses against backdoor attacks. The idea is straightforward; multi-layer approaches are to capture different levels of features, from simple patterns in lower layers to complex abstractions in higher layers, therefore providing more comprehensive extraction. We plan to look into this direction as well. %Previous studies, such as those by Wang et al.~\cite{wang2019neural} and Gao et al.~\cite{gao2019strip}, have demonstrated the effectiveness of multi-layer representations in detecting and mitigating backdoor attacks.
Asides from that there are less popular \NIID types \FB has not been applied to, we believe that \FB can be further improved in the following two direction. The first direction is to convert \FB into an unsupervised or semi-supervised method. One potential approach is to employ unsupervised contrastive learning~\cite{yang2021cade,fergusonefficient,bansal2023cleanclip} to train a self-supervised model that identifies malicious model updates through anomaly detection. The other direction is to further improve the design of buffer layer. One possibility is to use enhanced representation learning to improve the effectiveness of the buffer layer in \FB. For instance, existing work~\cite{CrowdGuard,MESAS} found that representation learning from multiple layers rather than PLRs only can strengthen defenses against backdoor attacks. We plan to look into this direction as well.%While some research has explored this direction~\cite{yang2021cade,fergusonefficient,bansal2023cleanclip}, their applicability on \NIIDs in FL remains unknown and difficult to predict as well. On the contrary, we consider model distillation~\cite{gou2021knowledge} may be a promising technique for this purpose. Recent studies~\cite{zhu2023adfl,zhang2024badcleaner} have used model distillation to create robust student models that inherit the defense capabilities of the corresponding teacher model against backdoor attacks. We plan to look into this direction.
% chen2020simple,radford2021learning,yang2021cade,fergusonefficient,bansal2023cleanclip
% CrowdGuard,MESAS,wang2019neural,wang2019neural

